Generating Transferable and Stealthy Adversarial Patch via Attention-guided Adversarial Inpainting

Adversarial patch attacks can fool the face recognition (FR) models via small patches. However, previous adversarial patch attacks often result in unnatural patterns that are easily noticeable. Generating transferable and stealthy adversarial patches that can efficiently deceive the black-box FR models while having good camouflage is challenging because of the huge stylistic difference between the source and target images. To generate transferable, natural-looking, and stealthy adversarial patches, we propose an innovative two-stage attack called Adv-Inpainting, which extracts style features and identity features from the attacker and target faces, respectively and then fills the patches with misleading and inconspicuous content guided by attention maps. In the first stage, we extract multi-scale style embeddings by a pyramid-like network and identity embeddings by a pretrained FR model and propose a novel Attention-guided Adaptive Instance Normalization layer (AAIN) to merge them via background-patch cross-attention maps. The proposed layer can adaptively fuse identity and style embeddings by fully exploiting priority contextual information. In the second stage, we design an Adversarial Patch Refinement Network (APR-Net) with a novel boundary variance loss, a spatial discounted reconstruction loss, and a perceptual loss to boost the stealthiness further. Experiments demonstrate that our attack can generate adversarial patches with improved visual quality, better stealthiness, and stronger transferability than state-of-the-art adversarial patch attacks and semantic attacks.

==> table5.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
\centering
  % \small
  % \tiny
\scriptsize    
\begin{tabular}{C{1.7cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}}
    \toprule
    Dataset & \multicolumn{4}{c}{LFW Dastaset} & \multicolumn{4}{c}{CelebA Dataset} & \multicolumn{4}{c}{FFHQ Dataset} \\   
    \cmidrule(rl){1-1}   \cmidrule(rl){2-5}  \cmidrule(rl){6-9}   \cmidrule(rl){10-13}  
    Victim Model  & ArcFace &  CosFace & MobFace & FaceNet & ArcFace & CosFace & MobFace & FaceNet & ArcFace & CosFace & MobFace & FaceNet  \\
    \midrule
    FGSM          & 87.55 & 8.26  & 3.75   & 10.92  & 89.45 & 4.56  & 6.14  & 8.44   & 92.43 & 8.64  & 5.60 & 10.32 \\
    PGD           & 98.73 & 13.45 & 11.80  & 12.60  & 94.56 & 12.57 & 9.90  & 13.50  & 95.45 & 10.64 & 8.85 & 12.45 \\
    C\&W          & 97.65 & 15.53 & 11.92  & 13.45  & 95.67 & 14.56 & 11.74 & 14.62  & 89.65 & 12.55 & 10.60 & 16.48\\
    MI-FGSM       & 95.48 & 16.55 & 16.27  & 14.52  & 98.90 & 15.89 & 8.23  & 15.30  & 98.20 & 15.35 & 10.24 & 13.25\\
    \midrule
    Adv-Glasses   & 47.43 & 3.55  & 4.60   & 8.20  & 45.43 & 2.41  & 5.67  & 9.10  & 43.43 & 13.23 & 14.60 & 12.20 \\
    Adv-Hat       & 76.46 & 9.40  & 3.10   & 4.80  & 75.23 & 14.54 & 8.56  & 4.74  & 56.43 & 23.40 & 22.10 & 14.21 \\
    TIDIM         & 89.68 & 25.48 & 24.88  & 32.56 & 88.34 & 27.86 & 21.77 & 22.53 & 85.38 & 25.40 & 24.60 & 32.52 \\   
    Gen-AP        & 75.65 & 22.56 & 19.90  & 8.20  & 82.45 & 21.34 & 24.40 & 25.82 & 81.75 & 32.56 & 29.90 & 12.20 \\
    SMAP          & 89.33 & 29.89 & 23.56  & 27.64 & 88.56 & 30.35 & 27.88 & 29.57 & 92.45 & 34.67 & 26.75 & 28.32  \\
    \midrule
    SemanticAdv   & 88.54 & 8.90  & 13.92  & 5.87  & 88.5  & 22.45 & 19.42 & 9.02  & 84.34 & 18.21 & 13.19 & 7.88 \\    
    Adv-Makeup    & 85.79 & 13.47 & 19.01  & 8.80  & 85.73 & 21.60 & 14.60 & 9.50 & 86.70 & 23.41 & 16.01 & 10.70\\
    Adv-Attribute & 86.36 & 28.70 & 26.50  & 25.90 & 86.36 & 23.52 & 25.65 & 31.80 & 84.45 & 28.72 & 22.52 & 31.45\\
    \midrule
   Ours w.o. AAIN & 89.57 & 29.78 & 28.12  & 34.58 & 83.67 & 29.46 & 24.15 & 36.17& 88.50 & 25.68 & 26.21 & 35.60\\
   Ours w.o. APT  & 90.55 & 35.71 & 30.82  & 37.41 & 84.56 & 34.45 & 33.05 & 38.20& 95.52 & 37.46 & 33.42 & 40.60\\
   Adv-Inpainting & 92.34 & \textbf{40.64} & \textbf{35.50}  & \textbf{42.95} & 93.40  & \textbf{37.10} & \textbf{38.36} & \textbf{42.30} & 95.45 & \textbf{37.97} & \textbf{35.45} &\textbf{42.40} \\
    \bottomrule
    \end{tabular}%
    % \vspace{1em}
  \caption{The attack success rates (\%) of impersonation attacks for the different face recognition models on the LFW and CelebA datasets. We chose the ArcFace model as the white-box model to train our models and evaluate the transferability of the other three FR models. We compare our attack with gradient-based, patch-based, and semantic-based attacks respectively.} 
  \label{tab:ASRonMobface}% 
\end{table}%


==> table6.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
\centering
  % \small
  % \tiny
\scriptsize    
\begin{tabular}{C{1.7cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}C{0.56cm}}
    \toprule
    Dataset & \multicolumn{4}{c}{LFW Dastaset} & \multicolumn{4}{c}{CelebA Dataset} & \multicolumn{4}{c}{FFHQ Dataset} \\   
    \cmidrule(rl){1-1}   \cmidrule(rl){2-5}  \cmidrule(rl){6-9}   \cmidrule(rl){10-13}  
    Victim Model  & ArcFace &  CosFace & MobFace & FaceNet & ArcFace & CosFace & MobFace & FaceNet & ArcFace & CosFace & MobFace & FaceNet  \\
    \midrule
    FGSM          & 87.55 & 8.26  & 3.75   & 10.92  & 89.45 & 4.56  & 6.14  & 8.44   & 92.43 & 8.64  & 5.60 & 10.32 \\
    PGD           & 98.73 & 13.45 & 11.80  & 12.60  & 94.56 & 12.57 & 9.90  & 13.50  & 95.45 & 10.64 & 8.85 & 12.45 \\
    C\&W          & 97.65 & 15.53 & 11.92  & 13.45  & 95.67 & 14.56 & 11.74 & 14.62  & 89.65 & 12.55 & 10.60 & 16.48\\
    MI-FGSM       & 95.48 & 16.55 & 16.27  & 14.52  & 98.90 & 15.89 & 8.23  & 15.30  & 98.20 & 15.35 & 10.24 & 13.25\\
    \midrule
    Adv-Glasses   & 47.43 & 3.55  & 4.60   & 8.20  & 45.43 & 2.41  & 5.67  & 9.10  & 43.43 & 13.23 & 14.60 & 12.20 \\
    Adv-Hat       & 76.46 & 9.40  & 3.10   & 4.80  & 75.23 & 14.54 & 8.56  & 4.74  & 56.43 & 23.40 & 22.10 & 14.21 \\
    TIDIM         & 89.68 & 25.48 & 24.88  & 32.56 & 88.34 & 27.86 & 21.77 & 22.53 & 85.38 & 25.40 & 24.60 & 32.52 \\   
    Gen-AP        & 75.65 & 22.56 & 19.90  & 8.20  & 82.45 & 21.34 & 24.40 & 25.82 & 81.75 & 32.56 & 29.90 & 12.20 \\
    SMAP          & 89.33 & 29.89 & 23.56  & 27.64 & 88.56 & 30.35 & 27.88 & 29.57 & 92.45 & 34.67 & 26.75 & 28.32  \\
    \midrule
    SemanticAdv   & 88.54 & 8.90  & 13.92  & 5.87  & 88.5  & 22.45 & 19.42 & 9.02  & 84.34 & 18.21 & 13.19 & 7.88 \\    
    Adv-Makeup    & 85.79 & 13.47 & 19.01  & 8.80  & 85.73 & 21.60 & 14.60 & 9.50 & 86.70 & 23.41 & 16.01 & 10.70\\
    Adv-Attribute & 86.36 & 28.70 & 26.50  & 25.90 & 86.36 & 23.52 & 25.65 & 31.80 & 84.45 & 28.72 & 22.52 & 31.45\\
    \midrule
   Ours w.o. AAIN & 89.57 & 29.78 & 28.12  & 34.58 & 83.67 & 29.46 & 24.15 & 36.17& 88.50 & 25.68 & 26.21 & 35.60\\
   Ours w.o. APT  & 90.55 & 35.71 & 30.82  & 37.41 & 84.56 & 34.45 & 33.05 & 38.20& 95.52 & 37.46 & 33.42 & 40.60\\
   Adv-Inpainting & 92.34 & \textbf{40.64} & \textbf{35.50}  & \textbf{42.95} & 93.40  & \textbf{37.10} & \textbf{38.36} & \textbf{42.30} & 95.45 & \textbf{37.97} & \textbf{35.45} &\textbf{42.40} \\
    \bottomrule
    \end{tabular}%
    % \vspace{1em}
  \caption{The attack success rates (\%) of impersonation attacks for the different face recognition models on the LFW and CelebA datasets. We chose the ArcFace model as the white-box model to train our models and evaluate the transferability of the other three FR models. We compare our attack with gradient-based, patch-based, and semantic-based attacks, respectively.} 
  \label{tab:ASRonFacenet}% 
\end{table}%

